On Quantifying Qualitative Geospatial Data: A Probabilistic Approach

Living in the era of data deluge, we have witnessed a web content explosion, largely due to the massive availability of User-Generated Content (UGC). In this work, we specifically consider the problem of geospatial information extraction and representation, where one can exploit diverse sources of information (such as image and audio data, text data, etc), going beyond traditional volunteered geographic information. Our ambition is to include available narrative information in an effort to better explain geospatial relationships: with spatial reasoning being a basic form of human cognition, narratives expressing such experiences typically contain qualitative spatial data, i.e., spatial objects and spatial relationships. To this end, we formulate a quantitative approach for the representation of qualitative spatial relations extracted from UGC in the form of texts. The proposed method quantifies such relations based on multiple text observations. Such observations provide distance and orientation features which are utilized by a greedy Expectation Maximization-based (EM) algorithm to infer a probability distribution over predefined spatial relationships; the latter represent the quantified relationships under user-defined probabilistic assumptions. We evaluate the applicability and quality of the proposed approach using real UGC data originating from an actual travel blog text corpus. To verify the quality of the result, we generate grid-based maps visualizing the spatial extent of the various relations.

==> conclusions2.tex <==
\section{Conclusions} 
\label{sec:conclusions}

The increase in the amount of available UGC data provides a unique opportunity for the generation of rich datasets in geographical information science.
In this work, we provide a quantitative approach for the representation of qualitative spatial relations extracted from such data, based on training probabilistic models. 
The proposed scheme returns estimates of uncertain object locations based on distance and orientation features, which are described by human reporters in relation to other 
known object locations. To achieve this desiderata, we propose a greedy learning algorithm based on the Expectation Maximization (EM) framework to train probabilistic models 
over spatial relationships; here, we restrict our attention on GMM models. %The results are visualized using a spatial grid for indicating probable object locations. 

The proposed approach seems to be promising in terms of efficiency, with attractive results for the representation of spatial relationships. Distance and orientation features 
tend to describe all spatial relations that were extracted from user generated texts in an informative way. Moreover, our probabilistic approach seems to be robust in handling 
any uncertainties, which characterize observations in crowd-sourced text data.

The directions for future work are as follows. A critical aspect in our work is the availability of qualitative data, i.e., the more examples are available, 
the better the quantitative representation of the relation will be. We are currently investigating targeted Web search for POI pairs to collect more spatial 
relationship instances to overall refine the current location estimates. This data fusion is similar to the approach used in surveying engineering when computing 
an unknown location based on distance and angle observations to known locations.
Finally, we will investigate existing techniques for the automatic extraction of POIs and spatial relationship information from texts.

==> intro.tex <==
%!TEX root = paper.tex
\section{Introduction} 
\label{sec:introduction}

During the last decade, we have witnessed an explosion in the amount and variety of on-line content available on the Web. Sophisticated analysis of such User Generated Content (UGC) 
has become an important issue in many cutting edge research fields such as geographical information science. In this work, our goal is to take advantage of such Volunteered Geographic Information (VGI) 
in geospatial data analysis. In particular, when applied to the geospatial domain, this translates to massively collecting and sharing knowledge in order to ultimately model and chart the world. 
With spatial reasoning being a basic form of human cognition, narratives expressing such experiences typically contain spatial knowledge. We formulate a quantitative approach for the representation 
of qualitative spatial relations extracted from UGC in the form of texts. In this context, by using only qualitative spatial information, there is no precision to the extent 
of quantitative information involved and hence such information is usually cheaper to obtain. In contrast, quantitative information is the standard type of data used in virtually 
all applications dealing with geospatial content, where high precision is required. 
%\textbf{Define qualitative vs. quantitative relations?}

To achieve this, our approach follows a probabilistic path: the proposed method quantifies qualitative relations as probability measures based 
on crowdsourced multiple observations contained in texts. Each observation is roughly quantified using a spatial feature vector comprising distance 
and orientation. Then, a greedy Expectation Maximization-based (EM) method is used to train a probability distribution. The latter represents the quantified 
spatial relationships under a probabilistic framework, i.e., it provides a set of random variables (spatial feature vector) that have certain probability density 
functions (PDFs) associated with them, for a specific spatial relation.

As a motivational example we could consider the sentence; \textit{``Big Ben is the nickname for the great bell of the clock at the north end of the Palace of Westminster''}. 
In this case, we want to quantify what people imply when they say \textit{``North''} in terms of distance and direction features. 
Having quantified \textit{``North''} in this context and knowing the location of either \textit{``Big Ben''} or \textit{``Palace of Westminster''} will allow us to infer 
possible locations for the other. Eventually, by collecting more observations in the form of \textit{``Big Ben is the great bell of the clock next to 
the Palace of Westminster''}, we will be able to refine the location. Overall, we will be able to locate spatial objects that otherwise could not be geocoded. 
Figure~\ref{fig:intuition} illustrates the underlying idea by relating our observation-based approach to the triangulation problem from surveying engineering, where an unknown 
location is determined by “observing” known locations. $P_i$, $P_j$ and $P_k$ represent known locations that are used to compute several unknown locations ($P_x$ and $P_y$) based on distance and angle observations.

% \begin{figure}[htbp]
% \includegraphics[width=\columnwidth]{drawings/intuition.png} \caption{Intuitive Problem Formalization} 
% \label{fig:intuition} 
% \end{figure}

\begin{figure}[htbp]
	\includegraphics[width=3.2in,height=1.8in]{drawings/intuition.png} \caption{Intuitive Problem Formalization} 
	\label{fig:intuition}  
\end{figure}

The outline of the remainder of this work is as follows. Section~\ref{sec:related_work} discusses related work. Section~\ref{sec:contribution} discusses the specific qualitative data involved and introduces the 
spatial feature vectors used for quantification, while Section~\ref{sec:statmodeling} introduces the tools necessary to derive quantification in the form of PDFs for the spatial 
relationships. Section~\ref{sec:experimentation} validates the proposed approach by means of “mapping” the obtained quantified relationships and using a similarity metric to assess the iterative quantification process. 
Finally, Section~\ref{sec:conclusions} presents conclusions and directions for future work.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%FROM EDBT2013%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% 
% 
% % The introduction essentially expands on the abstract (stepwise refinement). It has 3 sections (3 is always a good number when you present concepts).
% % You present and motivate the problem in more detail. Give background information. Why is this important? What are some real-world issues that we try to solve? 
% % Second, you briefly introduce the solutions that are out there and solve the problem already, i.e., related work in a nutshell.
% % Third, you introduce your solution, i.e., what are the important points of the solution your propose to solve the problem.
% % Say also how you will evaluate your solution. This is especially important for algorithmic papers, i.e., will it be experimental evaluation or theoretical.
% % The final part of this section is always the same you present the outline of the paper using more or less the following wording.
% %\textbf{qualitative vs quantitative}
% 
% With the proliferation of the Internet as the primary medium for data publishing and information exchange, we have seen 
% an explosion in the amount of online content available on the Web. Thus, in addition to professionally-produced 
% material offered freely on the Internet, Internet users tend to make multimedia content available online 
% to everyone. The volumes of such User-Generated 
% Content (UGC) are already staggering and constantly growing. Here, our goal is to take advantage of this explosion in Volunteered Geographic 
% Information (VGI). In particular, when applied to the geospatial domain, this translates to massively collecting and sharing knowledge to ultimately digitize the world. 
% %
% With \emph{spatial reasoning} being a basic form of human cognition for problem solving, narratives expressing such experiences typically contain 
% spatial knowledge, i.e., configurations among distinct spatial objects that are typically expressed in terms of qualitative spatial relationships.
% %
% Consequently, extraction, analysis and representation of spatial relationships existing in UGC has become an important issue in geographical information science. 
% In this work, a quantitative approach for the representation of qualitative spatial relations extracted from UGC in the form of texts is formulated. 
% Essentially, we want to quantify in terms of distance and direction as to what people imply when they say ``near'' or ``north''.
% % how to get from narratives to spatial relationships
% %Spatial relations have been classified into several types, including direction relations that describe order in space (e.g., north, north-east), topological relations that describe neighborhood and incidence (e.g., inside, overlap), ordinal relations that describe inclusion (ordinal relations are a subset of topological relations), and metric relations (e.g., near, far) \cite{Guting}. 
% %
% %Quantiative vs. qualitative
% In the context of user-generated content, by using only qualitative spatial information, there is no precision to the extent of 
% quantitative information involved and hence such information is usually cheaper to obtain.
% %
% In contrast, quantitative information is the standard type of data used in virtually all applications dealing with geospatial content, where high precision is required. 
% 
% % in this paper
% % - extract spatial relationships from texts
% % - inflate them
% % - quantiy them
% % why? think of advanced geocoding in which an unknown location is known only in terms of qualitative data with respect to a known relation
% 
% % from abstract
% %In this work, a quantitative approach for the representation of qualitative spatial relations extracted from UGC in the form of texts is formulated. Training probabilistic models, the proposed method quantifies qualitative relations based on crowdsourced multiple observations contained in texts, e.g., instances of ``near''. Each observation is quantified using distance and orientation features and a greedy learning algorithm based on Expectation Maximization (EM) is used to train Gaussian Mixture Models (GMMs). The latter represent the quantified spatial relationships under a probabilistic framework. The applicability and quality of the proposed approach is assessed in an experimental evaluation involving an actual travel blog text corpus. To verify the result quality, we generate grid-based ``maps'' visualizing the spatial extent of the various relations.
% 
% In this paper, we study the problem of \emph{quantifying qualitative spatial relations} based on large sample sizes extracted from user-generated
%  narratives (travel blogs). Essentially, this will allow us quantify observations with respect to spatial data given in qualitative terms. Consider the example 
% ``\textbf{Big Ben} is the nickname for the great bell of the clock \emph{at the north end} of the \textbf{Palace of Westminster}'', having quantified \emph{North} 
% in this context and knowing the location of either ``Big Ben'' or ``Palace of Westminster'' will allow us to infer possible locations for the other. Eventually, 
% by collecting more observations in the form of ``\textbf{Big Ben} is the great bell of the clock \emph{next to} the \textbf{Palace of Westminster}'', we will be 
% able to refine the location. Overall, we will be able to locate spatial objects that otherwise could not be geocoded. 
% %
% Figure~\ref{fig:intuition} illustrates the underlying idea by relating our observation-based approach to the triangulation problem from surveying 
% engineering, where an unknown location is determined by ``observing'' known locations. $P_i$ and $P_j$ represent known locations that are used to
% compute several unknown locations based on distance and angle observations.
% %
% \begin{figure}[htbp]
% 	\includegraphics[width=\columnwidth]{drawings/intuition.png} \caption{Intuitive Problem Formalization} 
% 	\label{fig:intuition} 
% \end{figure}
% 
% 
% %These two reports refer to the same object and the same location in the London. However, neither of these reports can specify the exact location of the object \textit{``Big Ben''}, nor do they mention a special hint, like same street names, that could reveal the exact location of the object. We would like to represent such reports in a way that it enables efficient analyses and representation of uncertain locations based on observations from UGT. For instance, the representation must enable us to locate objects or events in a given geographical region e.g. around Westminster Palace. Likewise, it should enable us to determine similarity between reports based on their spatial properties; e.g., we should be able to determine that the above reports might refer to the same location by fusioning information that comes from two different spatial relations. 
% 
% %Overall, our primary motivation in studying the aforementioned problem comes from designing solutions to support applications where the real world is being monitored (potentially using a variety of sensing technologies) to support tasks such as location prediction, situation assessment and decision making. Such applications abound in a variety of domains including rural and surveying Engineering , homeland security, emergency response, command and control, process monitoring and business activity monitoring. Our particular interest lies in the domain of survey engineering and mapping using UGT. We already alluded to the usefulness of spatial reasoning over free text in the example above. Such solutions are useful in a variety of other application scenarios. For instance, such a system could create maps of objects or events that are described by internet users. 
% 
% %An example Another problem that could be solved using such a system is the existance of disputed areas. There are huge archives that describe disputed areas all over the world, but nobody can bound them in an accurate way. So, such a system could parse all text archives and constract stohastic maps that could disambiguate all disputed areas. In our project, we are building a quantitative spatial relation tool to enable us to perform spatial analysis over two datasets: (1) Travelblogs, e.g narratives about people's trips around the worls (2) Google querries. We deeply believe that techniques such as ours can benefit a very broad class of applications where free text is used to describe events. Our goal in this paper is to model spatial relations in a quantitative framework in order to represent uncertain object locations specified in reports. 
% 
% %extraction of spatial relationships from text
% 
% This task will be achieved by training probabilistic models. The proposed method quantifies qualitative relations based on 
% crowdsourced multiple observations contained in texts, e.g., instances of \emph{Near}. Each observation is roughly quantified 
% using a spatial feature vector comprising \emph{distance} and \emph{orientation}. A greedy learning algorithm based on Expectation Maximization (EM) 
% is used to train Gaussian Mixture Models (GMMs). The latter represents the quantified spatial relationships under a probabilistic framework, i.e., 
% it provides a set of random variables (spatial feature vector) that have certain probability density functions (pdfs) associated with them, 
% for a specific spatial relation. 
% 
% The applicability and quality of the proposed approach is assessed in an experimental evaluation involving an actual travel blog text corpus for the specific area of London, UK. 
% %
% To verify the result quality, we generate grid-based ``maps'' visualizing the spatial extent of the various relations; this construction provides further interpretation of the results.
% In addition, we assess divergence for each spatial relationship between a baseline model and the output model after each step of training so as to provide a means to 
% assess the output quality and to optimize the method. Moreover, assessing divergence allows reasoning about the similarity between two spatial relationships, e.g., \emph{NextTo} and \emph{Near}.
% 
% %outline
% The outline of the remainder of this work is as follows. 
% %
% Section~\ref{sec:related_work} discusses related work. 
% %
% Section~\ref{sec:contribution} discusses the specific qualitative data involved and introduces the spatial feature vectors used for quantification, while 
% %
% Section~\ref{sec:statmodeling} introduces the tools necessary to derive quantification in the form of probability functions for the spatial relationships.
% %
% Section~\ref{sec:experimentation} validates the proposed approach by means of ``mapping'' the obtained quantified relationships and using a similarity metric to assess the iterative quantification process. 
% %
% Finally, Section~\ref{sec:conclusions} presents conclusions and directions for future work.
% 
% 






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% % \section{Introduction} 
% % \label{sec:introduction}
% % 
% % 
% % % The introduction essentially expands on the abstract (stepwise refinement). It has 3 sections (3 is always a good number when you present concepts).
% % % You present and motivate the problem in more detail. Give background information. Why is this important? What are some real-world issues that we try to solve? 
% % % Second, you briefly introduce the solutions that are out there and solve the problem already, i.e., related work in a nutshell.
% % % Third, you introduce your solution, i.e., what are the important points of the solution your propose to solve the problem.
% % % Say also how you will evaluate your solution. This is especially important for algorithmic papers, i.e., will it be experimental evaluation or theoretical.
% % % The final part of this section is always the same you present the outline of the paper using more or less the following wording.
% % %\textbf{qualitative vs quantitative}
% % The term spatial knowledge refers to configurations among distinct spatial entities. As an example of the use of spatial knowledge representations in everyday life, 
% % consider subway maps. These maps do not display the shapes and sizes of the stations or quantitative distances between stations, but they contain line and point data and preserve spatial relations and intersects. 
% % Qualitative knowledge representation does not require an intermediate domain in which scale is defined, but comparisons are performed directly in the represented domain; in the domain of spatial knowledge, object 
% % locations are compared through spatial relations [Freksa]. Spatial relations have been classified into several types, including direction relations that describe order in space (e.g., north, north-east), 
% % topological relations that describe neighborhood and incidence (e.g., inside, overlap), ordinal relations that describe inclusion (ordinal relations are a subset of topological relations), and 
% % distance relations (e.g., near, far). These types of spatial relations have been studied independently or in association with each other. There are several reasons for following a qualitative approach 
% % to spatial knowledge representation: a)the precision of quantitative representations is not always desirable b) the input and the output of spatial processes is often qualitative rather than quantitative 
% % c) qualitative knowledge is usually cheaper.
% % 
% % On the other hand quantitative is always there. We always need precise information about thei real relation, e.g. 
% % distance and orientation from one to the others and vice verce, between objects in space. Several sciences including transportation, ecology, public safety, public health, climatology, and location-based 
% % services need a quantitative representation of spatial knowledge.
% % 
% % In this paper, we study the problem of representing uncertain location information about real world objects or points of interest (POIs) that are described in user generated text (UGT). 
% % As a motivating example about the reason we have to deal with this problem we can consider the excerpts from two real reports anybody can find in world wide web:
% % \begin{itemize}
% % 	\item ``\textit{Big Ben is the nickname for the great bell of the clock \textbf{at the north end} of the Palace of Westminster}'' 
% % 	\item ``\textit{Big Ben is the great bell of the clock \textbf{next to} the Palace of Westminster}'' 
% % \end{itemize}
% % 
% % These two reports refer to the same object and the same location in the London. However, neither of these reports can specify the exact location of 
% % the object \textit{``Big Ben''}, nor do they mention a special hint, like same street names, that could reveal the exact location of the object. 
% % We would like to represent such reports in a way that it enables efficient analyses and representation of uncertain locations based on observations from UGT. 
% % For instance, the representation must enable us to locate objects or events in a given geographical region e.g. around Westminster Palace. Likewise, it should enable us to determine 
% % similarity between reports based on their spatial properties; e.g., we should be able to determine that the above reports might refer to the same location by fusioning information 
% % that comes from two different spatial relations. Our primary motivation in studying the aforementioned problem comes from designing solutions to support applications where the real 
% % world is being monitored (potentially using a variety of sensing technologies) to support tasks such as location prediction, situation assessment and decision making. Such applications 
% % abound in a variety of domains including rural and surveying Engineering , homeland security, emergency response, command and control, process monitoring and business activity monitoring. 
% % Our particular interest lies in the domain of survey engoneering and mapping using UGT. We already alluded to the usefulness of spatial reasoning over free text in the example above. 
% % Such solutions are useful in a variety of other application scenarios. For instance, such a system could create maps of objects or events that are described by internet users. 
% % More specifically we will be able to place on the map, objects that are not geocoded but are described based on other geocoded objects. Another problem that could be solved using such a 
% % system is the existance of disputed areas. There are huge archives that describe disputed areas all over the world, but nobody can bound them in an accurate way. So, such a system could parse 
% % all text archives and constract stohastic maps that could disambiguate all disputed areas. In our project, we are building a quantitative spatial relation tool to enable us to perform spatial 
% % analysis over two datasets: (1) Travelblogs, e.g narratives about people's trips around the worls (2) Google querries. We deeply believe that techniques such as ours can benefit a very broad 
% % class of applications where free text is used to describe events. Our goal in this paper is to model spatial relations in a quantitative framework in order to represent uncertain object locations 
% % specified in reports. \\
% % 
% % To support spatial analyses on free text reports, we need to project the spatial properties of the spatial relation described in the report onto the domain. In this paper, 
% % we model uncertain object spatial relations as sets of random variables that have certain probability density functions (pdfs) associated with them. Our approach is based on the assumption 
% % that people report object locations based on certain landmarks, e.g., objects that are already geocoded. Let be a 2-dimensional physical space in which the objects described in the reports are immersed. 
% % Landmarks correspond to significant spatial objects such as buildings, streets, intersections, regions, cities, areas, etc. embedded in the space. Spatial location of objects specified in those reports
% %  can be mapped into spatial relations.\\
% % \begin{figure}
% % 	\includegraphics[width=3.2in,height=2.2in]{drawings/intuition.pdf} \caption{Intuitive Problem Formalization} \label{fig:intuition} 
% % \end{figure}
% % 
% % %outline
% % The outline of the remainder of this work is as follows. Section ~\ref{sec: related_work} discusses related work. Section ~\ref{sec: contribution} describes the contribution of 
% % your work. Section ~\ref{sec: experimentation} validates the proposed approach by means of an empirical performance study. Finally, Section ~\ref{sec: conclusions} presents conclusions 
% % and directions for future work.
